Simulating Anisoplanatic Turbulence by Sampling Inter-modal and Spatially Correlated Zernike Coefficients

Simulating atmospheric turbulence is an essential task for evaluating turbulence mitigation algorithms and training learning-based methods. Advanced numerical simulators for atmospheric turbulence are available, but they require evaluating wave propagation which is computationally expensive. In this paper, we present a propagation-free method for simulating imaging through turbulence. The key idea behind our work is a new method to draw inter-modal and spatially correlated Zernike coefficients. By establishing the equivalence between the angle-of-arrival correlation by Basu, McCrae and Fiorino (2015) and the multi-aperture correlation by Chanan (1992), we show that the Zernike coefficients can be drawn according to a covariance matrix defining the correlations. We propose fast and scalable sampling strategies to draw these samples. The new method allows us to compress the wave propagation problem into a sampling problem, hence making the new simulator significantly faster than existing ones. Experimental results show that the simulator has an excellent match with the theory and real turbulence data.

==> TeX/customFigureMacros.tex <==
% ===========================================================
% Definitions, commands and environnments for drawing figures
%
% Vivek Goyal
% based on work by
% Ivana Jovanovic, Patrick Vandewalle, Olivier Roy - 2005
% ===========================================================

% --------
% PACKAGES
% --------
%\RequirePackage{amsmath}
%\RequirePackage{amssymb}
\RequirePackage{xspace}
\RequirePackage{bbm}
\RequirePackage{ifthen}
%\RequirePackage{pstricks}
%\RequirePackage{pst-plot}
%\RequirePackage{algo}
%\RequirePackage{epsfig}
%\RequirePackage{latexsym}
%\RequirePackage{subfigure}

% --------------------
% PSTRICKS DEFINITIONS
% --------------------
% Upsampling operation (reference point at the center of the circle)
% Parameter #1: upsampling factor
\def\upsampling#1{

    \pscircle(0,0){0.5}
    \psline{->}(-0.15,-0.25)(-0.15,0.25)
    \rput(0.15,0){#1}

}

% Downsampling operation (reference point at the center of the circle)
% Parameter #1: downsampling factor
\def\downsampling#1{

    \pscircle(0,0){0.5}
    \psline{<-}(-0.15,-0.25)(-0.15,0.25)
    \rput(0.15,0){#1}

}

% Sampling operation (reference point at the center of the box)
% Parameter #1: sampling period
% This is a quick-and-dirty job; definitely less beautiful than other macros.
\def\sampler#1{

    \psframe(-1,-0.5)(1,0.5)
    \psline{-}(-0.6,-0.2)(-0.2,-0.2)
    \psline{-}(0.2,-0.2)(0.6,-0.2)
    \psline{-}(-0.2,-0.2)(0.1,0.1)
    \rput(-0.3,0.3){#1}

}

% Discrete-to-continuous operation (reference point at the center of the box)
% (Generation of weighted Dirac train)
% Parameter #1: sampling period
% This is a quick-and-dirty job; definitely less beautiful than other macros.
\def\diracTrain#1{

    \psframe(-1,-0.5)(1,0.5)
    \psline{-}(-0.8,0)(0.8,0)
    \psline{->}(-0.6,0)(-0.6,-0.45)
    \psline{->}(-0.3,0)(-0.3,-0.3)
    \psline{->}( 0.0,0)( 0.0, 0.4)
    \psline{->}( 0.3,0)( 0.3, 0.4)
    \psline{->}( 0.6,0)( 0.6,-0.35)
    \rput(0.3,-0.2){#1}

}

% Filter (reference point at the center of the box)
% Parameter #1: filter label
\def\filter#1{

    \psframe(-1,-0.5)(1,0.5)
    \rput(0,0){#1}

}

\def\shortfilter#1{

    \psframe(-0.75,-0.5)(0.75,0.5)
    \rput(0,0){#1}

}

% Filter (reference point at the center of the box)
% Parameter #1: filter label
\def\widefilter#1{

    \psframe(-2,-0.5)(2,0.5)
    \rput(0,0){#1}

}

% Sum (reference point at the center of the circle)
\def\sumsymbol{

    \pscircle(0,0){0.25}
    \rput(0,0){$+$}

}

% Analysis part of a filter bank channel (reference point at the begining of the channel)
% Parameter #1: analysis filter label
% Parameter #2: downsampling factor
\def\analysis#1#2{

    \psline{-}(0,0)(0.5,0)
    \rput(1.5,0){\filter{#1}}
    \psline{-}(2.5,0)(3,0)
    \rput(3.5,0){\downsampling{#2}}
    \psline{-}(4,0)(4.5,0)
}

% Analysis part of a filter bank channel (reference point at the begining of the channel)
% Parameter #1: analysis filter label
% Parameter #2: downsampling factor
\def\wideanalysis#1#2{

    \psline{-}(0,0)(0.5,0)
    \rput(2.5,0){\widefilter{#1}}
    \psline{-}(4.5,0)(5,0)
    \rput(5.5,0){\downsampling{#2}}
    \psline{-}(6,0)(6.5,0)
}

% Synthesis part of a filter bank channel (reference point at the begining of the channel)
% Parameter #1: synthesis filter label
% Parameter #2: upsampling factor
\def\synthesis#1#2{

    \psline{-}(0,0)(0.5,0)
    \rput(1,0){\upsampling{#2}}
    \psline{-}(1.5,0)(2,0)
    \rput(3,0){\filter{#1}}
    \psline{-}(4,0)(4.5,0)
}

% Filter bank channel (reference point at the begining of the channel)
% Parameter #1: analysis filter label
% Parameter #2: synthesis filter label
% Parameter #3: down/upsampling factor
\def\filterbankchannel#1#2#3{

    \rput(0,0){\analysis{#1}{#3}}
    \rput(4.5,0){\synthesis{#2}{#3}}

}

% Two channel filter bank (reference point at the begining of the filter bank)
% Parameter #1: lowpass analysis filter label
% Parameter #2: lowpass synthesis filter label
% Parameter #3: highpass analysis filter label
% Parameter #4: highpass synthesis filter label

\def\twochannelfilterbank#1#2#3#4{

    % Input
    \psline{*-}(0,0)(0.5,0)
    \psline{-}(0.5,-0.75)(0.5,0.75)

    % Highpass branch
    \rput(0.5,0.75){\filterbankbranch{#3}{#4}{2}}

    % Lowpass branch
    \rput(0.5,-0.75){\filterbankbranch{#1}{#2}{2}}

    % Output
    \psline{->}(9.5,0.75)(9.5,0.25)
    \rput(9.5,0){\sumsymbol}
    \psline{->}(9.5,-0.75)(9.5,-0.25)
    \psline{-*}(9.75,0)(10.25,0)

}




% Parameter #1: filter label
% Parameter #2: sampling factor
% Parameter #3: delay
\def\mybranch#1#2#3{
    \psline{-}(0,0)(0.5,0)
    \rput(1,0){\upsampling{#2}}
    \psline{-}(1.5,0)(2,0)
    \rput(2.75,0){\shortfilter{#3}}
    \psline{-}(3.5,0)(4,0)
    \rput(5,0){\filter{#1}}
    \psline{-}(6,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8,0)
}


\def\mybranchA#1#2{
    \psline{-}(-0.5,0)(0.5,0)
    \rput(1,0){\upsampling{#2}}
    \psline{-}(1.5,0)(4,0)
    \rput(5,0){\filter{#1}}
    \psline{-}(6,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8.5,0)
}


\def\mybranchB#1#2#3{
    \psline{-}(0,0)(0.5,0)
    \rput(1.5,0){\filter{#1}}
    \psline{-}(2.5,0)(3,0)
    \rput(3.5,0){\upsampling{#2}}
    \psline{-}(4,0)(4.5,0)
    \rput(5.25,0){\shortfilter{#3}}
    \psline{-}(6,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8,0)
}


\def\mybranchC#1#2{
    \psline{-}(-0.5,0)(0.5,0)
    \rput(1.5,0){\filter{#1}}
    \psline{-}(2.5,0)(3,0)
    \rput(3.5,0){\upsampling{#2}}
    \psline{-}(4,0)(6.5,0)
    \rput(7,0){\downsampling{#2}}
    \psline{-}(7.5,0)(8.5,0)
}
